MMCORE: MultiModal COnnection with Representation Aligned Latent Embeddings

We present MMCORE, a unified framework designed for multimodal image generation and editing. MMCORE leverages a pre-trained Vision-Language Model (VLM) to predict semantic visual embeddings via learnable query tokens, which subsequently serve as conditioning signals for a diffusion model. This streamlined design effectively transfers the rich understanding and reasoning capabilities of VLMs into the visual generation process. By obviating the need for deep fusion between autoregressive and diffusion models or training from scratch, MMCORE significantly reduces computational overhead while maintaining high-fidelity synthesis. MMCORE seamlessly integrates text-to-image synthesis with interleaved image generation, demonstrating robust multimodal comprehension in complex scenarios such as spatial reasoning and visual grounding. Comprehensive evaluations indicate that MMCORE consistently outperforms state-of-the-art baselines across a broad spectrum of text-to-image and single/multi-image editing benchmarks.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}
\sun{experiment results from Yichun's doc}
We validate our design choices using GPT-4o and Doubao scores to assess semantic alignment and visual quality.

\paragraph{\textbf{Design of the VLM-DiT Connector}}
We analyze the impact of connector depth (2-6 layers) and capacity. As shown in Table~\ref{tab:ablation_connector}, a shallow 2-layer mapping performs poorly (0.6791). Increasing depth to 6 layers significantly boosts performance to 0.7843, and expanding channel width yields further gains (0.8104). This confirms that a high-capacity projector is essential for bridging the modality gap.

% \subsection{Fine-tuning Strategies: Full vs. Parameter-Efficient}
\paragraph{\textbf{Fine-tuning Strategies: Full vs. Parameter-Efficient}}
We compare three integration strategies: Connector-Only, LoRA, and Full Fine-tuning. Tuning only the connector yields the lowest results, indicating DiT weights must adapt. While LoRA (rank=128) closes the gap, full fine-tuning achieves the best convergence and generation quality ($>0.85$). Additionally, fusing intermediate VLM states (Mixed) outperforms using only the last hidden state.

% \subsection{Effectiveness of Supervised Fine-Tuning (SFT)}
\paragraph{\textbf{Effectiveness of Supervised Fine-Tuning (SFT)}}
Table~\ref{tab:ablation_sft} compares extended pretraining against our two-stage SFT strategy. Extending pretraining (50k steps) shows diminishing returns, plateauing at $\sim$0.81. In contrast, a short 2k-step SFT phase dramatically boosts the score to \textbf{0.8585}, and \textbf{0.87+} with larger batches. SFT proves indispensable for aligning outputs with human aesthetics.

\paragraph{\textbf{Diffusion-forcing vs denoise last only}} We study how different choices of training targets affect diffusion forcing in image sequences. In one variant, we treat every image in the sequence (except the leading image) as a diffusion generation target. In the other variant, we supervise diffusion only on the final image, using all preceding text and images purely as conditioning context. We train on an image–text interleaved dataset comprising 3M sequences sourced from videos and web data, and evaluate on our in-house image-editing benchmark. As shown in Table~\ref{tab:ablation diff forcing}, diffusion forcing utilizes the data more effectively under a fixed token budget: for the same sequence length and total number of training tokens, a larger fraction of tokens receive direct training signal, leading to improved performance.

%-------------------------------------------------------------------------
% Table 1: Ablation on Connector & Strategy (Modified: No Row Column)
%-------------------------------------------------------------------------
\begin{table}[t]
\centering
\caption{\textbf{Ablation on Connector Architecture and Fine-tuning Strategy.} We evaluate the impact of connector depth and different tuning methods. Metrics are reported on our internal test set (Dreambench) for text-to-image generation.}
\label{tab:ablation_connector}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c l c c}
\toprule
Model Setup & Connector Depth & Tuning Strategy & GPT-4o $\uparrow$ & Doubao $\uparrow$ \\
\midrule
Baseline (SeedVLM V2) & 2 Layers & Connector Only & 0.6791 & 0.7276 \\
 & 3 Layers & Connector Only & 0.7490 & 0.7910 \\
 & 6 Layers & Connector Only & 0.7843 & 0.8396 \\
 & 6 Layers (+128ch) & Connector Only & \textbf{0.8104} & \textbf{0.8487} \\
\midrule
LoRA & 6 Layers & LoRA (Rank=128) & 0.8423 & 0.8779 \\
Ours & 6 Layers & Full Fine-tune & \textbf{0.8528} & \textbf{0.8738} \\
\bottomrule
\end{tabular}
}
\end{table}

%-------------------------------------------------------------------------
% Table 2: Ablation on SFT
%-------------------------------------------------------------------------
\begin{table}[t]
\centering
\caption{\textbf{Impact of Training Stages (Pretrain vs. SFT).} Comparing extended pretraining against the proposed two-stage SFT strategy. ``EMA'' denotes Exponential Moving Average.}
\label{tab:ablation_sft}
\begin{tabular}{l l c c}
\toprule
Stage & Config / Steps & GPT-4o $\uparrow$ & Doubao $\uparrow$ \\
\midrule
\multirow{2}{*}{\textbf{Pretrain}} & 20k Steps & 0.7975 & 0.8504 \\
 & 50k Steps (EMA) & 0.8139 \small{(+0.016)} & 0.8531 \\
\midrule
\multirow{3}{*}{\textbf{SFT}} & + Mix SFT 3k & 0.8304 & 0.8599 \\
 & + SFT 2k & 0.8585 \small{(+0.044)} & 0.8915 \\
 & \textbf{+ SFT 2k (Best)} & \textbf{0.8784} & \textbf{0.9043} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Impact of different interleave training strategies} Comparing diffusion forcing and denoising only the last image in the sequence.}
\label{tab:ablation diff forcing}
\begin{tabular}{l c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Doubao}\\
\cline{2-3}
 & \textit{Alignment} $\uparrow$& \textit{Consistency} $\uparrow$\\
\hline
Diffusion forcing & 0.7148 & 0.3462 \\
Denoise last only & 0.6787 & 0.3203 \\
\bottomrule
\end{tabular}
\end{table}


==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiment}

In this section, we elaborate on our setup of experiments, including evaluation sets and metrics.

%\subsection{Hello World}
\subsection{Evaluation.}
We first collected a few hundred testing images, based on both real and generated images. These test image sets include a wide range of editing operations. To be specific, in addition to common stylization, add, replace, and delete, we also include many instructive motions from camera, object shift, scene shot change, etc. which provide us a good guide on how well the model is performed in general user usage, rather than biased towards a few cases. 

For evaluation metrics, we consider the CLIP image simlairty and CLIP direction score metric proposed in InstructPix2Pix~\citep{brooks2023instructpix2pix}, and the GPT scores with the same GPT-4o model mentioned in HQEdit~\citep{hui2024hqedit} for quick machine-based evaluation. 
To make the evaluation more solid for product applications, we also adopt a set of human evaluations for the final quality check, shown in Fig.~\ref{fig:performance}, including a 0-5 scoring standard in three aspects: 1) instruction response, which evaluates whether the model responded to the instruction; 2) image consistency, whether the model preserved the identity after change; 3) image quality, which evaluates whether the model generates images with good quality without artifacts.  To summarize, we also provide satisfactory rates from 0-100, e.g. Usability Rate and Satisfaction Rate, as the percentage of satisfied edited images for a final summarization of model performance to benchmark different methods. Usability Rate means the results have minor non-satisfaction points (<3), and Satisfactory Rate means having 0 non-satisfaction points. In Fig.~\ref{fig:performance}, we set the max rate for Usability and Satisfaction to 60\% and 30\% respectively for better visualization due to our strict standards.  This metric aligns the standards from our T2I~\cite{seedream3.0} models and user feedback from our previous release versions, which has proven to be effective in online user performance evaluation.


\subsection{Comparisons}
 As shown in Fig.~\ref{fig:quati}, we show the quantitative comparison results of auto-machine evaluation with a few SoTA algorithms such as Step1x~\cite{liu2025step1x}, Gemini~\cite{gemini2.0} and GPT4o~\cite{hurst2024gpt}. The better models are located at the right top of the figure. 
To be fair on numbers, we run the open-source model with 1024 resolution for Step1x, and run others with their website chatting window with 4 times and choose the visually best one. For non-responded image queries, especially GPT4o and Gemini, we omit the score in evaluation. We have conducted extensive experiments with comparisons, and found that such evaluation metrics are well aligned with human feeling. 

We compare the current version with our multiple previous versions: SeedEdit1.0~\cite{shi2024seededit}, SeedEdit1.5 (by adding more data sources), and SeedEdit1.6 which were the data merging strategy and reward modeling added.
%
% Compared with our previous versions SeedEdit1.0~\cite{shi2024seededit}, in this report, we named adding more data sources as SeedEdit1.5, and adding the data merging strategy and reward modeling as SeedEdit1.6. 
 %
 This ablates different strategies as discussed in Sec.~\ref{subsec:data}.
 Our final model is represented by the yellow dots, namely SeedEdit3.0, which significantly improves over our previous versions and also outperforms other methods such as Gemini and Step1x in both metrics. For GPT-4o, it is located at the right bottom, which demonstrates that it has better prompt and instruction-following ability, while we find it has relatively weak image consistency, as demonstrated by CLIP image similarity and face similarity, which significantly impacts its human satisfaction rate as evaluated previously.

 The overall performance curve based on human evaluation has been illustrated in Fig.~\ref{fig:performance}, which shows that SeedEdit3.0 has the best trade-off across multiple metrics,  yielding the highest satisfaction rate for users. More importantly, we are comparably much faster, as it takes only 10-15s per image, compared to 50-60s per image for GPT-4o. 

Fig.~\ref{fig:quali} illustrates more comparison examples between our SeedEdit3.0 and SoTA models, where we further confirm the conclusion of our evaluation; we use results from single set of CFGs rather than picking from multiple ones. Additionally, we also notice a recent open source model: Step1X~\cite{liu2025step1x}, and find that it is difficult to compare directly with these commercial models, especially in real image quality, editing intention following, and understanding. 

\subsection{Ablation Study}


\section{Conclusion}
In this report, we have introduced SeedEdit3.0, which significantly improves our previous versions in terms of real image performance, face/id preservation, text editing quality, prompt understanding, dynamic motion, etc. We presented an efficient data curation
pipeline that allows it to scale editing data  effectively; while a joint learning method was introduced to further enhance image consistency, which is particularly important for real-world applications. This results in a high-performance image editing system, which hopefully can be well used and adopted by all users to enrich their creativity. 

==> sections/relatedwork.tex <==
\section{Related Work}
% \peng{Xiaochen, please help this part}
We briefly review a few recent methods for instructive editing, covering the two most important topics: diffusion model methods and data set creation.  

metaqueries, metacanvas, 

\paragraph{\textbf{Instruct Editing Methods}}
% \peng{xiaochen data : training free methods can be simply referred, major mention some training methods such as adobe's, step1x, gpt and gemini etc. }

Existing methods using diffusion models for image editing can be primarily categorized into two groups: training-free approaches and training approaches. The training-free method controls the generation of images in the denoising process, by inverting the diffusion process~\cite{mokady2023null,nie2023blessing,feng2025dit4edit,lin2024schedule} and attention crontrol~\cite{hertz2022prompt,cao2023masactrl,tumanyan2023plug}. Although fast and low-cost, they all suffer from inferior content preservation and low editing accuracy, e.g., inconsistency with either the input image or the target descriptions. 

To achieve the best editing quality, it is widely acknowledged that retraining a diffusion model is necessary. Early training-based approaches~\cite{wang2023instructedit, brooks2023instructpix2pix, zhang2023magicbrush, shi2024seededit} train diffusion-based editing models on synthesized image editing datasets. Later works focus on novel model architectures for better instruction-image interaction~\cite{huang2024smartedit, yang2024mastering, yu2024anyedit, zhao2024ultraedit}. Recently, unified image generation and editing framework has attracted more and more attention. OmniGen~\cite{xiao2024omnigen}, Transfusion~\cite{zhou2024transfusion},  and Mogao~\cite{liao2025mogao} jointly model text and images within a single transformer to achieve unified representations. DreamEngine~\cite{chen2025multimodal}, MetaQueries~\cite{pan2025transfer} and Step1X-Edit~\cite{liu2025step1x} connect the text and image latent features of Multimodal LLM (MLLM) to the diffusion decoder, leveraging MLLM's strong capabilities in understanding and reasoning. By joint vision-language training, Gemini 2.0~\cite{gemini2.0} and GPT-4o~\cite{hurst2024gpt} have demonstrated strong performance in following instruction and generating consistent images. In this paper, we will compare model with SeedEdit, GPT-4o and Gemini on real image editing tasks.

\paragraph{\textbf{Dataset Creation}} 
% \peng{xiaochen data : omniedit, anyedit, instrutive move etc. }

One of the major challenges in training an instruction-based image editing model is the lack of large-scale datasets that have high-quality image editing pairs with corresponding instructions. Early approaches like Magicbrush~\cite{zhang2023magicbrush} construct datasets by manually labeling image pairs, which is not scalable and can hardly cover all types of image editing. InstructPix2Pix~\cite{brooks2023instructpix2pix} and HIVE~\cite{zhang2024hive} leverage GPT-3~\cite{brown2020language} and Prompt2Prompt~\cite{hertz2022prompt} to generate image editing pairs. HQ-EDIT~\cite{hui2024hqedit} and UltraEdit~\cite{zhao2024ultraedit} further push the quality of this data synthesis pipeline by using more powerful foundation models such as GPT-4V~\cite{hurst2024gpt} and DALL-E 3~\cite{dalle3}. To ensure the diversity and quality of the synthesized data, Seed-Edit~\cite{shi2024seededit} combines different regeneration techniques and sampling hyperparameters and applies importance sampling to obtain diverse and high-quality training examples. Synthesized data has a strong bias towards the underlying generative models. To handle real images, \cite{wei2024omniedit,sheynin2024emu} train multiple expert models, each specializing in a different editing task, to generate a large, high-resolution, multi-aspect ratio dataset. Our data curation pipeline, as described in Sect.~\ref{subsec:data}, inherits all the merits of existing pipelines, e.g., including both synthesized and real images of high quality, multiple sources, and different sizes, utilizing LLM/VLM to enrich the editing instructions and to ensure precise alignment between the paired images and their corresponding instructions, designing a reliable data assessment process to control the data quality, etc.

% Existing methods using diffusion models for image editing can be primarily categorized into three groups: training-free approaches, inference-time fine-tuning approaches, and data-driven training approaches. 

% Firstly, the training-free method controls image generation in the denoising process. Text-based methods refine input texts [] or enhance text embeddings [] to enable conceptual modifications and user instruction following. \cite{mokady2023null}[null-text, SDE-Drag, DiT4Edit, Schedule Your Edit] apply solver inversion (e.g., DDIM and DPM-solver inversion) to construct the noise latent space of input images and regenerate the target images conditioned on the text prompts. Attention control methods [Prompt-to-Prompt, masactrl, Plug-and-play] manipulate the attention features during the reverse diffusion steps to achieve the editing goals and content consistency. Although fast and low-cost, training-free methods suffer from inferior content preservation and low editing accuracy, e.g., inconsistency with either the input image or the target descriptions.

% Step1X-Edit
% Gemini 2.0
% Janus: Decoupling visual encoding for unified multimodal understanding and generation.
% Janus-pro: Unified multimodal understanding and generation with data and model scaling
%  Show-o: One single transformer to unify multimodal understanding and generation


